The Role of Twist in Kinked Flux Rope Emergence and Delta-Spot Formation

It has been observationally well established that the magnetic configurations most favorable for producing energetic flaring events reside in delta-spots, a class of sunspots defined as having opposite polarity umbrae sharing a common penumbra. They are frequently characterized by extreme compactness, strong rotation and anti-Hale orientation. Numerous studies have shown that nearly all of the largest solar flares originate in delta-spots, making the understanding of these structures a fundamental step in predicting space weather. Despite their important influence on the space environment, surprisingly little is understood about the origin and behavior of delta-spots. In this paper, we perform a systematic study of the behavior of emerging flux ropes to test a theoretical model for the formation of delta-spots: the kink instability of emerging flux ropes. We simulated the emergence of highly twisted, kink-unstable flux ropes from the convection zone into the corona, and compared their photospheric properties to those of emerged weakly twisted, kink-stable flux ropes. We show that the photospheric manifestations of the emergence of highly twisted flux ropes closely match the observed properties of delta-spots, and we discuss the resulting implications for observations. Our results strongly support and extend previous theoretical work that suggested that the kink instability of emerging flux ropes is a promising candidate to explain delta-spot formation, as it reproduces their key characteristics very well.

==> figures_file.tex <==
\newpage
\clearpage
\begin{figure*}
\centering\includegraphics[scale=0.5, trim=0.0cm 0.0cm 0.0cm 0.0cm,clip=true]{atmosphere.pdf}
\caption{Stratified atmosphere used in flux emergence simulations. The mass density (blue), pressure (orange) and temperature (red) are scaled by their photospheric ($x = 0$) values. Shown in black is the magnetic pressure profile for the $\zeta=1$ flux rope. The convection zone is located at $x/H_p<0$, the temperature minimum region at $0<x/H_p<12$, and the corona begins at $x/H_p=25$, being separated from the temperature minimum portion of the atmosphere by a short transition region.}
\label{fig:atmosphere}
\end{figure*}

\newpage 


\begin{figure*}
\centering\includegraphics[scale=0.29, trim=0.0cm 1.0cm 4.0cm 0.0cm,clip=true]{iso05_1.pdf}
\centering\includegraphics[scale=0.32, trim=4.0cm 1.0cm 5.0cm 3.0cm,clip=true]{iso05_above1.pdf}
\centering\includegraphics[scale=0.29, trim=0.0cm 1.0cm 4.0cm 0.0cm,clip=true]{iso05_2.pdf}
\centering\includegraphics[scale=0.32, trim=4.0cm 1.0cm 5.0cm 3.0cm,clip=true]{iso05_above2.pdf}
\centering\includegraphics[scale=0.29, trim=0.0cm 1.0cm 4.0cm 0.0cm,clip=true]{iso05_3.pdf}
\centering\includegraphics[scale=0.32, trim=4.0cm 1.0cm 5.0cm 3.0cm,clip=true]{iso05_above3.pdf}
\centering\includegraphics[scale=0.29, trim=0.0cm 1.0cm 4.0cm 0.0cm,clip=true]{iso05_4.pdf}
\centering\includegraphics[scale=0.32, trim=4.0cm 1.0cm 5.0cm 3.0cm,clip=true]{iso05_above4.pdf}
%\vspace{-0.9cm}
\caption{Isosurfaces (yellow) of $B=1\;\mathrm{kG}$ during the $\zeta=0.5$ flux rope's rise through the convection zone. The photosphere is located at $x=0$. Left: Seen from the side, with color shading representing temperature, plotted on a linear scale, and mass density, plotted on a log scale. Right: Seen from above.}
\label{fig:isosurfaces05}
\end{figure*}

\begin{figure*}
\centering\includegraphics[scale=0.5, trim=0.0cm 0.0cm 0.0cm 0.0cm,clip=true]{striations.pdf}
\caption{Close-up of isosurface shown in Figures \ref{fig:isosurfaces05}c,d with several field lines overplotted on the striations visible along the isosurface.}
\label{fig:striations}
\end{figure*}

\begin{figure*}
\centering\includegraphics[scale=0.32, trim=1.0cm 1.0cm 5.5cm 1.0cm,clip=true]{twist05_bx1.pdf}
\centering\includegraphics[scale=0.32, trim=3.0cm 1.0cm 5.5cm 1.0cm,clip=true]{twist05_bx_line.pdf}
\centering\includegraphics[scale=0.32, trim=1.0cm 1.0cm 5.5cm 1.0cm,clip=true]{twist05_bx3.pdf}
\centering\includegraphics[scale=0.32, trim=3.0cm 1.0cm 5.5cm 1.0cm,clip=true]{twist05_bx_vec_zoom.pdf}
\centering\includegraphics[scale=0.5, trim=0.0cm 0.0cm 0.0cm 0.0cm,clip=true]{colorbar.pdf}
\caption{Vertical field, $B_x$, on photosphere during the $\zeta=0.5$ simulation, saturated at $\pm500\;\mathrm{G}$. The middle state of the simulation (panel b) is shown with the flux weighted centers of mass (red circles connected with a line), while the final state of the simulation (panel d) has the horizontal field $\vecB_h$ as colored vectors overplotted on the greyscale.}
\label{fig:bx0}
\end{figure*}
\begin{figure*}
\centering\includegraphics[scale=0.25, trim=0.0cm 0.0cm 0.0cm 0.0cm,clip=true]{twist05_beg1.pdf}
\centering\includegraphics[scale=0.25, trim=0.0cm 0.0cm 0.0cm 0.0cm,clip=true]{twist05_beg2.pdf}
\centering\includegraphics[scale=0.25, trim=0.0cm 0.0cm 0.0cm 0.0cm,clip=true]{twist05_mid.pdf}
\centering\includegraphics[scale=0.25, trim=0.0cm 0.0cm 0.0cm 0.0cm,clip=true]{twist05_end.pdf}
\caption{Field lines, overplotted on photospheric magnetograms, at various stages of the $\zeta=0.5$ simulation. In a) and b) field lines, colored by $B_y$, are seen from the side and above, respectively. In d) field lines are shown at the final state of the simulation, colored by $v_x$.}
\label{fig:fieldlines0}
\end{figure*}


\begin{figure*}
\centering\includegraphics[scale=0.29, trim=0.0cm 1.0cm 4.0cm 0.0cm,clip=true]{iso1_1.pdf}
\centering\includegraphics[scale=0.32, trim=4.0cm 1.0cm 5.0cm 3.0cm,clip=true]{iso1_above1.pdf}
\centering\includegraphics[scale=0.29, trim=0.0cm 1.0cm 4.0cm 0.0cm,clip=true]{iso1_2.pdf}
\centering\includegraphics[scale=0.32, trim=4.0cm 1.0cm 5.0cm 3.0cm,clip=true]{iso1_above2.pdf}
\centering\includegraphics[scale=0.29, trim=0.0cm 1.0cm 4.0cm 0.0cm,clip=true]{iso1_3.pdf}
\centering\includegraphics[scale=0.32, trim=4.0cm 1.0cm 5.0cm 3.0cm,clip=true]{iso1_above3.pdf}
\centering\includegraphics[scale=0.29, trim=0.0cm 1.0cm 4.0cm 0.0cm,clip=true]{iso1_4.pdf}
\centering\includegraphics[scale=0.32, trim=4.0cm 1.0cm 5.0cm 3.0cm,clip=true]{iso1_above4.pdf}
\caption{Same as Figure \ref{fig:isosurfaces05} for $\zeta=1$}
\label{fig:isosurfaces1}
\end{figure*}

\begin{figure*}
\centering\includegraphics[scale=0.32, trim=1.0cm 1.0cm 5.5cm 1.0cm,clip=true]{twist1_bx1.pdf}
\centering\includegraphics[scale=0.32, trim=3.0cm 1.0cm 5.5cm 1.0cm,clip=true]{twist1_bx_line.pdf}
\centering\includegraphics[scale=0.32, trim=1.0cm 1.0cm 5.5cm 1.0cm,clip=true]{twist1_bx3.pdf}
\centering\includegraphics[scale=0.32, trim=3.0cm 1.0cm 5.5cm 1.0cm,clip=true]{twist1_bx_vec_zoom.pdf}
\centering\includegraphics[scale=0.5, trim=0.0cm 0.0cm 0.0cm 0.0cm,clip=true]{colorbar.pdf}
\caption{Same as Figure \ref{fig:bx0}, for the $\zeta=1$ case. Primary/secondary polarities are denoted by blue/yellow arrows in panel b).}
\label{fig:bx1}
\end{figure*}

\begin{figure*}
\centering\includegraphics[scale=0.25, trim=0.0cm 0.0cm 0.0cm 0.0cm,clip=true]{twist1_beg1.pdf}
\centering\includegraphics[scale=0.25, trim=0.0cm 0.0cm 0.0cm 0.0cm,clip=true]{twist1_beg2.pdf}
\centering\includegraphics[scale=0.25, trim=0.0cm 0.0cm 0.0cm 0.0cm,clip=true]{twist1_mid.pdf}
\centering\includegraphics[scale=0.25, trim=0.0cm 0.0cm 0.0cm 0.0cm,clip=true]{twist1_end.pdf}
\caption{Field lines, overplotted on photospheric magnetograms, at various stages of the $\zeta=1$ simulation. In a) and b) field lines, colored by $B_y$, are seen from the side and above, respectively. In d) field lines are shown at the final state of the simulation, colored by $v_x$.}
\label{fig:fieldlines1}
\end{figure*}


\begin{figure*}
\centering\includegraphics[scale=0.3, trim=0.0cm 1.0cm 4.0cm 0.0cm,clip=true]{forpaper1.5/iso15_1.pdf}
\centering\includegraphics[scale=0.32, trim=4.0cm 1.0cm 5.0cm 3.0cm,clip=true]{forpaper1.5/iso15_above1.pdf}
\centering\includegraphics[scale=0.3, trim=0.0cm 1.0cm 4.0cm 0.0cm,clip=true]{forpaper1.5/iso15_2.pdf}
\centering\includegraphics[scale=0.32, trim=4.0cm 1.0cm 5.0cm 3.0cm,clip=true]{forpaper1.5/iso15_above2.pdf}
\centering\includegraphics[scale=0.3, trim=0.0cm 1.0cm 4.0cm 0.0cm,clip=true]{forpaper1.5/iso15_3.pdf}
\centering\includegraphics[scale=0.32, trim=4.0cm 1.0cm 5.0cm 3.0cm,clip=true]{forpaper1.5/iso15_above3.pdf}
\centering\includegraphics[scale=0.3, trim=0.0cm 1.0cm 4.0cm 0.0cm,clip=true]{forpaper1.5/iso15_4.pdf}
\centering\includegraphics[scale=0.32, trim=4.0cm 1.0cm 5.0cm 3.0cm,clip=true]{forpaper1.5/iso15_above4.pdf}
\caption{Same as Figure \ref{fig:isosurfaces05} for $\zeta=1.5$}
\label{fig:isosurfaces15}
\end{figure*}

\begin{figure*}
\centering\includegraphics[scale=0.32, trim=1.0cm 1.0cm 5.5cm 1.0cm,clip=true]{forpaper1.5/twist15_bx1.pdf}
\centering\includegraphics[scale=0.32, trim=3.0cm 1.0cm 5.5cm 1.0cm,clip=true]{forpaper1.5/twist15_bx2.pdf}
\centering\includegraphics[scale=0.32, trim=1.0cm 1.0cm 5.5cm 1.0cm,clip=true]{forpaper1.5/twist15_bx_line.pdf}
\centering\includegraphics[scale=0.32, trim=3.0cm 1.0cm 5.5cm 1.0cm,clip=true]{forpaper1.5/twist15_bx4.pdf}
\centering\includegraphics[scale=0.32, trim=1.0cm 1.0cm 5.5cm 1.0cm,clip=true]{forpaper1.5/twist15_bx_vec_zoom.pdf}
\caption{Same as Figure \ref{fig:bx0}, for the $\zeta=1.5$ case. Primary/secondary polarities are denoted by blue/yellow arrows in panel c).}
\label{fig:bx1.5}
\end{figure*}

\begin{figure*}
\centering\includegraphics[scale=0.25, trim=0.0cm 0.0cm 0.0cm 0.0cm,clip=true]{forpaper1.5/twist15_beg1.pdf}
\centering\includegraphics[scale=0.25, trim=0.0cm 0.0cm 0.0cm 0.0cm,clip=true]{forpaper1.5/twist15_beg2.pdf}
\centering\includegraphics[scale=0.25, trim=0.0cm 0.0cm 0.0cm 0.0cm,clip=true]{forpaper1.5/twist15_mid1.pdf}
\centering\includegraphics[scale=0.25, trim=0.0cm 0.0cm 0.0cm 0.0cm,clip=true]{forpaper1.5/twist15_mid2.pdf}
\centering\includegraphics[scale=0.25, trim=0.0cm 0.0cm 0.0cm 0.0cm,clip=true]{forpaper1.5/twist15_end.pdf}
\caption{Field lines, overplotted on photospheric magnetograms, at various stages of the $\zeta=1.5$ simulation. In a) and b) field lines, colored by $B_y$, are seen from the side and above, respectively. In e) field lines are shown at the final state of the simulation, colored by $v_x$.}
\label{fig:fieldlines1.5}
\end{figure*}

\begin{figure*}
\centering\includegraphics[scale=0.3, trim=0.0cm 1.0cm 4.0cm 0.0cm,clip=true]{iso2_1.pdf}
\centering\includegraphics[scale=0.32, trim=4.0cm 1.0cm 5.0cm 3.0cm,clip=true]{iso2_above1.pdf}
\centering\includegraphics[scale=0.3, trim=0.0cm 1.0cm 4.0cm 0.0cm,clip=true]{iso2_2.pdf}
\centering\includegraphics[scale=0.32, trim=4.0cm 1.0cm 5.0cm 3.0cm,clip=true]{iso2_above2.pdf}
\centering\includegraphics[scale=0.3, trim=0.0cm 1.0cm 4.0cm 0.0cm,clip=true]{iso2_3.pdf}
\centering\includegraphics[scale=0.32, trim=4.0cm 1.0cm 5.0cm 3.0cm,clip=true]{iso2_above3.pdf}
\centering\includegraphics[scale=0.3, trim=0.0cm 1.0cm 4.0cm 0.0cm,clip=true]{iso2_4.pdf}
\centering\includegraphics[scale=0.32, trim=4.0cm 1.0cm 5.0cm 3.0cm,clip=true]{iso2_above4.pdf}
\caption{Same as Figure \ref{fig:isosurfaces05} for $\zeta=2$}
\label{fig:isosurfaces2}
\end{figure*}

\begin{figure*}
\centering\includegraphics[scale=0.32, trim=1.0cm 1.0cm 5.5cm 1.0cm,clip=true]{twist2_bx1.pdf}
\centering\includegraphics[scale=0.32, trim=3.0cm 1.0cm 5.5cm 1.0cm,clip=true]{twist2_bx2.pdf}
\centering\includegraphics[scale=0.32, trim=1.0cm 1.0cm 5.5cm 1.0cm,clip=true]{twist2_bx_line.pdf}
\centering\includegraphics[scale=0.32, trim=3.0cm 1.0cm 5.5cm 1.0cm,clip=true]{twist2_bx4.pdf}
\centering\includegraphics[scale=0.32, trim=1.0cm 1.0cm 5.5cm 1.0cm,clip=true]{twist2_bx_vec_zoom.pdf}
\caption{Same as Figure \ref{fig:bx0}, for the $\zeta=2$ case. Primary/secondary polarities are denoted by blue/yellow arrows in panels b) and c).}
\label{fig:bx2}
\end{figure*}

\begin{figure*}
\centering\includegraphics[scale=0.25, trim=0.0cm 0.0cm 0.0cm 0.0cm,clip=true]{twist2_beg1.pdf}
\centering\includegraphics[scale=0.25, trim=0.0cm 0.0cm 0.0cm 0.0cm,clip=true]{twist2_beg2.pdf}
\centering\includegraphics[scale=0.25, trim=0.0cm 0.0cm 0.0cm 0.0cm,clip=true]{twist2_mid1.pdf}
\centering\includegraphics[scale=0.25, trim=0.0cm 0.0cm 0.0cm 0.0cm,clip=true]{twist2_mid2.pdf}
\centering\includegraphics[scale=0.25, trim=0.0cm 0.0cm 0.0cm 0.0cm,clip=true]{twist2_end.pdf}
\centering\includegraphics[scale=0.25, trim=0.0cm 0.0cm 0.0cm 0.0cm,clip=true]{twist2_end2.pdf}
\caption{Field lines, overplotted on photospheric magnetograms, at various stages of the $\zeta=2$ simulation. In a) and b) field lines, colored by $B_y$, are seen from the side and above, respectively. In e) field lines are shown at the final state of the simulation, colored by $v_x$.}
\label{fig:fieldlines2}
\end{figure*}

\begin{figure*}
\centering\includegraphics[scale=0.29, trim=0.0cm 1.0cm 4.0cm 0.0cm,clip=true]{iso4_1.pdf}
\centering\includegraphics[scale=0.32, trim=4.0cm 1.0cm 5.0cm 3.0cm,clip=true]{iso4_above1.pdf}
\centering\includegraphics[scale=0.29, trim=0.0cm 1.0cm 4.0cm 0.0cm,clip=true]{iso4_2.pdf}
\centering\includegraphics[scale=0.32, trim=4.0cm 1.0cm 5.0cm 3.0cm,clip=true]{iso4_above2.pdf}
\centering\includegraphics[scale=0.29, trim=0.0cm 1.0cm 4.0cm 0.0cm,clip=true]{iso4_3.pdf}
\centering\includegraphics[scale=0.32, trim=4.0cm 1.0cm 5.0cm 3.0cm,clip=true]{iso4_above3.pdf}
\centering\includegraphics[scale=0.29, trim=0.0cm 1.0cm 4.0cm 0.0cm,clip=true]{iso4_4.pdf}
\centering\includegraphics[scale=0.32, trim=4.0cm 1.0cm 5.0cm 3.0cm,clip=true]{iso4_above4.pdf}
\caption{Same as Figure \ref{fig:isosurfaces05} for $\zeta=4$}
\label{fig:isosurfaces4}
\end{figure*}

\begin{figure*}
\centering\includegraphics[scale=0.32, trim=1.0cm 1.0cm 5.5cm 1.0cm,clip=true]{twist4_bx1.pdf}
\centering\includegraphics[scale=0.32, trim=3.0cm 1.0cm 5.5cm 1.0cm,clip=true]{twist4_bx2.pdf}
\centering\includegraphics[scale=0.32, trim=1.0cm 1.0cm 5.5cm 1.0cm,clip=true]{twist4_bx_line.pdf}
\centering\includegraphics[scale=0.32, trim=3.0cm 1.0cm 5.5cm 1.0cm,clip=true]{twist4_bx4.pdf}
\centering\includegraphics[scale=0.32, trim=1.0cm 1.0cm 5.5cm 1.0cm,clip=true]{twist4_bx_vec_zoom.pdf}
\caption{Same as Figure \ref{fig:bx0}, for the $\zeta=4$ case. Primary/secondary polarities are denoted by blue/yellow arrows in panels b) and c).}
\label{fig:bx4}
\end{figure*}
\begin{figure*}
\centering\includegraphics[scale=0.25, trim=0.0cm 0.0cm 0.0cm 0.0cm,clip=true]{twist4_beg1.pdf}
\centering\includegraphics[scale=0.25, trim=0.0cm 0.0cm 0.0cm 0.0cm,clip=true]{twist4_beg2.pdf}
\centering\includegraphics[scale=0.25, trim=0.0cm 0.0cm 0.0cm 0.0cm,clip=true]{twist4_knot.pdf}
\centering\includegraphics[scale=0.25, trim=0.0cm 0.0cm 0.0cm 0.0cm,clip=true]{twist4_knot_single.pdf}
\centering\includegraphics[scale=0.25, trim=0.0cm 0.0cm 0.0cm 0.0cm,clip=true]{twist4_mid1.pdf}
\centering\includegraphics[scale=0.25, trim=0.0cm 0.0cm 0.0cm 0.0cm,clip=true]{twist4_mid2.pdf}
\centering\includegraphics[scale=0.25, trim=0.0cm 0.0cm 0.0cm 0.0cm,clip=true]{twist4_end.pdf}
\centering\includegraphics[scale=0.25, trim=0.0cm 0.0cm 0.0cm 0.0cm,clip=true]{twist4_end2.pdf}
\caption{Field lines, overplotted on photospheric magnetograms, at various stages of the $\zeta=4$ simulation. In a) and b) field lines, colored by $B_y$, are seen from the side and above, respectively. In c), a single knotted field line is shown, with several other field lines shown wrapped up in the knotted field line in d). In g) field lines are shown at the final state of the simulation, colored by $v_x$.}
\label{fig:fieldlines4}
\end{figure*}
\begin{figure*}
\centering\includegraphics[scale=0.27, trim=0.0cm 0.0cm 0.0cm 0.0cm,clip=true]{twoFRs_fieldlines.pdf}
\centering\includegraphics[scale=0.27, trim=0.0cm 0.0cm 0.0cm 0.0cm,clip=true]{twoFRs_fieldlines_zoom.pdf}
\centering\includegraphics[scale=0.3, trim=1.0cm 1.7cm 6.0cm 0.7cm,clip=true]{twoFRs05.pdf}
\centering\includegraphics[scale=0.3, trim=1.0cm 1.7cm 6.0cm 0.7cm,clip=true]{twoFRs1.pdf}
\centering\includegraphics[scale=0.3, trim=1.0cm 1.7cm 6.0cm 0.7cm,clip=true]{twoFRs15.pdf}
\centering\includegraphics[scale=0.3, trim=1.0cm 1.7cm 6.0cm 0.7cm,clip=true]{twoFRs2.pdf}
\centering\includegraphics[scale=0.3, trim=0.0cm 1.7cm 6.0cm 0.7cm,clip=true]{twoFRs4.pdf}
\caption{a) Two flux ropes, with a peak field strength of $B_0=6.5\;\mathrm{kG}$, oriented at $\pm45^\circ$ to the vertical. b) Zoom in of a), with red arrows denoting example field lines which cross the photosphere twice. $B_x$ (greyscale) and $B_h$ (colored vectors) due to two flux ropes oriented at a $45^\circ$ angle to the vertical with c) $\zeta=0.5$, d) $\zeta=1$, e) $\zeta=1.5$, f) $\zeta=2$, g) $\zeta=4$. The color table applies to panels c-g.}
\label{fig:twoFRs}
\end{figure*}

\begin{figure*}
\centering\includegraphics[scale=0.45, trim=0.0cm 0.0cm 0.0cm 0.0cm,clip=true]{Separation_Distance.pdf}
\centering\includegraphics[scale=0.45, trim=0.0cm 0.0cm 0.0cm 0.0cm,clip=true]{Rotation_Angle.pdf}
\caption{Top: The distance between the flux weighted centers of mass, $|\textbf{L}_{com}|$. Bottom: The angle between the line connecting the flux weighted centers of mass and the $y$-axis, $\theta_{com}$ vs.\ time for each simulation. $t=0$ is defined as the instant a photospheric pixel first exceeds $B_x = 30\;\mathrm{G}$.}
\label{fig:seprot}
\end{figure*}
\begin{figure*}%[!p]
\centering\includegraphics[scale=0.45, trim=0.0cm 0.0cm 0.0cm 0.0cm,clip=true]{total_flux.pdf}
\centering\includegraphics[scale=0.45, trim=0.0cm 0.0cm 0.0cm 0.0cm,clip=true]{flux_emergence_rate_points.pdf}
\caption{Top: Unsigned scaled photospheric flux $\Phi_{sc}$ vs. time for each simulation. Bottom: Flux emergence rate vs.\ emerged flux, plotted following \citet{Norton17}}
\label{fig:flux}
\end{figure*}

\begin{figure*}
\centering\includegraphics[scale=0.35, trim=0.0cm 0.0cm 0.0cm 0.0cm,clip=true]{Mean_Jx.pdf}
\centering\includegraphics[scale=0.35, trim=0.0cm 0.0cm 0.0cm 0.0cm,clip=true]{Mean_abs_Jx.pdf}
\centering\includegraphics[scale=0.35, trim=0.0cm 0.0cm 0.0cm 0.0cm,clip=true]{Neutralization_Ratio.pdf}
\caption{Average signed vertical current density $\bar{J}_x$ (top), average unsigned current density $\overline{|J_x|}$ (middle) and current neutralization ratio $\mathcal{R}$ (bottom) as functions of time for each simulation.}
\label{fig:currents}
\end{figure*}


\newpage
\begin{figure*}
\centering\includegraphics[scale=0.3, trim=0.0cm 0.0cm 0.0cm 0.0cm,clip=true]{Mean_Alpha_normal.pdf}
\centering\includegraphics[scale=0.3, trim=0.0cm 0.0cm 0.0cm 0.0cm,clip=true]{Mean_Alpha.pdf}
\centering\includegraphics[scale=0.3, trim=0.0cm 0.0cm 0.0cm 0.0cm,clip=true]{Mean_Alpha_normal_ff.pdf}
\centering\includegraphics[scale=0.3, trim=0.0cm 0.0cm 0.0cm 0.0cm,clip=true]{Mean_Alpha_ff.pdf}
\caption{a) $\bar{\alpha_x}$ b) $\bar{\alpha}$ c) $\bar{\alpha}_{x,ff}$, d) $\bar{\alpha}_{ff}$, as functions of time for each simulation.}
\label{fig:alpha}
\end{figure*}

\newpage
\begin{figure*}
\centering\includegraphics[scale=0.38, trim=0.0cm 1.0cm 5.5cm 1.0cm,clip=true]{alphax1.pdf}
\centering\includegraphics[scale=0.38, trim=0.0cm 1.0cm 5.0cm 1.0cm,clip=true]{alpha1.pdf}
\centering\includegraphics[scale=0.38, trim=0.0cm 1.0cm 5.5cm 1.0cm,clip=true]{ffalphax1.pdf}
\centering\includegraphics[scale=0.38, trim=0.0cm 1.0cm 5.0cm 1.0cm,clip=true]{ffalpha1.pdf}
\caption{a) $\alpha_x$ b) $\alpha$, c) $\alpha_{x,ff}$, and d) $\alpha_{ff}$ for $\zeta=1$.}
\label{fig:alphas1}
\end{figure*}

\begin{figure}
\centering\includegraphics[scale=0.35, trim=0.0cm 0.0cm 0.0cm 0.0cm,clip=true]{MagE.pdf}
\centering\includegraphics[scale=0.35, trim=0.0cm 0.0cm 0.0cm 0.0cm,clip=true]{PotE.pdf}
\centering\includegraphics[scale=0.35, trim=0.0cm 0.0cm 0.0cm 0.0cm,clip=true]{FreeEnergy.pdf}
\caption{Top: Magnetic energy in the corona as a function of time, scaled by the initial magnetic energy in the whole volume. Middle: Potential energy in the corona as a function of time, scaled by the initial magnetic energy in the whole volume. Bottom: Free energy in the corona as a function of time, scaled by the initial magnetic energy in the whole volume.}
\label{fig:energy}
\end{figure}


